Probe-Me-Not: Protecting Pre-trained Encoders from Malicious Probing

Adapting pre-trained deep learning models to customized tasks has become a popular choice for developers to cope with limited computational resources and data volume. More specifically, probing--training a downstream head on a pre-trained encoder--has been widely adopted in transfer learning, which helps to prevent overfitting and catastrophic forgetting. However, such generalizability of pre-trained encoders raises concerns about the potential misuse of probing for harmful intentions, such as discriminatory speculation and warfare applications. In this work, we introduce EncoderLock, a novel applicability authorization method designed to protect pre-trained encoders from malicious probing, i.e., yielding poor performance on specified prohibited domains while maintaining their utility in authorized ones. Achieving this balance is challenging because of the opposite optimization objectives and the variety of downstream heads that adversaries can utilize adaptively. To address these challenges, EncoderLock employs two techniques: domain-aware weight selection and updating to restrict applications on prohibited domains/tasks, and self-challenging training scheme that iteratively strengthens resistance against any potential downstream classifiers that adversaries may apply. Moreover, recognizing the potential lack of data from prohibited domains in practical scenarios, we introduce three EncoderLock variants with different levels of data accessibility: supervised (prohibited domain data with labels), unsupervised (prohibited domain data without labels), and zero-shot (no data or labels available). We verify EncoderLock's effectiveness and practicality with a real-world pre-trained Vision Transformer (ViT) encoder from Facebook. These results underscore the valuable contributions EncoderLock brings to the development of responsible AI.

==> text/artifacts.tex <==
\newpage
\section{Artifact Appendix}

\subsection{Description and Requirements}

\subsubsection{How to Access}
Our artifacts include the source code to run the training and evaluation process of EncoderLock.

\subsubsection{Hardware Dependencies}
A GPU is highly recommended for testing the source code to ensure faster training and evaluation.

\subsubsection{Software Dependencies}
The required software includes Python 3.9 and PyTorch 1.12.

\subsubsection{Datasets}
Most of the datasets can be downloaded via \texttt{torchvision}. We also provide links to download the real-world datasets (i.e., ImageNette and Military Vehicle) in the README file and the main manuscript.

\subsection{Artifact Installation}
The artifacts run in a Python 3.9 environment. We recommend installing the required packages in an Anaconda environment using the \texttt{environment.yml} file.

\subsection{Experiment Workflow}
The experiment consists of three parts:

\begin{itemize}
    \item \textbf{Data and Model Preparation}: To run the experiment, we first need to prepare data from both the source domain and the target domain (synthetic dataset for the zero-shot EncoderLock). Additionally, we need a victim pre-trained encoder that performs well on the source domain but is vulnerable to malicious probing on the target domain.
    \item \textbf{EncoderLock Training}: In this stage, the user should fine-tune the encoder using the proposed method to obtain a modified encoder that resists malicious probing on the target domain.
    \item \textbf{EncoderLock Testing}: In this stage, the user needs to test the probing performance of the modified encoder on the target domain to demonstrate that the model is protected against probing.
\end{itemize}

\subsection{Major Claims}
We demonstrate the effectiveness of EncoderLock in protecting against malicious probing. The main results are presented in Table~\ref{tab: target ntl performance} and Table~\ref{tab: unsupervised encoderlock performance}. Specifically, you should observe that while the source domain experiences a slight degradation in testing accuracy, the target domain accuracy drops significantly after implementing EncoderLock.

\subsection{Evaluations}
\subsubsection{Experiment Cost}
Training EncoderLock usually takes from 0.1 to 6 GPU hours, varying depending on the GPU platform and the dataset.

\subsubsection{How To}
Please follow the steps in the \texttt{README.md} file included with the artifacts to run the evaluations.

\subsubsection{Execution}
We provide scripts to directly run all evaluations; you can find them under the \texttt{/tests/} directory.

\subsubsection{Customization}
Hyperparameters can be directly adjusted in the execution scripts.


==> text/formulation.tex <==
% \section{Problem Formulation} \label{sec: problem formulation}


==> text/motivation.tex <==
\section{Design Motivation and Objective} \label{sec: motivation}
\ruyi{merge section 3, 4. 4.3-->3.1, (3.2 3.3) 4.1+4.2-->5, multi-level--> section 5 and 3.3}
\subsection{Limitations in Non-transferable Learning} \label{sec: authorized transferability}
While IP protection traditionally defends against stealing model attributes such as its architecture, parameters, or hyperparameters, the rise of EaaS introduces another dimension: the need to prevent transfers to unauthorized domains. 
% For instance, it would be critical to deter the use of a pre-trained vehicle feature extractor for military weaponry vehicles.
Classical Non-transferable Learning (NTL)~\cite{wang2022non} 
addresses it by crafting specialized loss functions to reduce the generalization bound of the model. 
However, one may need more flexible solutions because such online services still require domain transferability for privileged users, such as system administrators, who will continuously update the service by frequently fine-tuning it on new data. 
Furthermore, commercially, EaaS providers can benefit by granting different levels of encoder transferability to users depending on their authorizations.
While ordinary users may be subject to transferability limitations, privileged users can exploit the encoder's full transfer learning capabilities. 
% Moreover, training multiple models tailored for various user levels can be prohibitively costly.
Thus, EaaS requires an easily controllable encoder to adjust transferability rather than restrict it during the training stage. 
For instance, in commercial recommendation systems, safeguarding the model being transferred by rival entities but maintaining its robust transferability for privileged users, such as system administrators or premium members, is crucial.
\ls{If I remebered correctly, the consensus is not to mention NTL too often???} 
\ruyi{Yes, we try to emphasize the difference between our \MyMethod versus previous NTL.}
\ls{be specific? This generalizability can be messed up with model generalization errors.}  
\ruyi{make it clearer here. the term generalization bound is used in the original paper.}
\ls{Here is an inconsistency. Based on Fig.\,\ref{fig: framework design}, it seems that a user can keep both authorized and unauthrized tasks.}
\ruyi{Try to make it clearer here. The authorized data, tasks is on the user side. The EaaS only limit the usage onto those tasks.}
\begin{table}[t]
    \caption{\textbf{\MyMethod properties---}Comparison with Non-transferable Learning (NTL)~\cite{wang2022non},  Model Barrier (MB)~\cite{wang2023model}.}
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule[0.6mm]
       & NTL~\cite{wang2022non} & MB~\cite{wang2023model} & \textbf{EL} (Ours)  \\
    \midrule
    Target-free   & \cmark  &\cmark & \cmark \\
    Sparsity  & \xmark  & \xmark & \cmark \\
    Robustness &  \xmark  & \xmark & \cmark \\
    Plug-and-Play  & \xmark & \cmark & \cmark \\
    Switch Flexibility & \xmark  & \xmark & \cmark \\
    Various Label Space   & \xmark  & \xmark & \cmark \\
    Real-world Encoder & \xmark  & \xmark & \cmark\\
    \bottomrule[0.6mm]
    \end{tabular}
    \label{tab: comparison with baselines}
\end{table}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/gradient-importance.pdf}
    \caption{\textbf{Visualization of weight importance in transfer learning---}The X-Y plane is for the weight matrix of the selected dense layer.
    The color and height of a peak indicate the importance of it to the model output.
    }
    \label{fig: motivation-dfa}
\end{figure}

In Table~\ref{tab: comparison with baselines}, we highlight the limitations of existing NTL methods by contrasting them with \MyMethod. 
Our novel approach specifically addresses these shortcomings, enhancing robustness against malicious fine-tuning of the model and introducing sparse updating for improved defense efficiency. 
While previous works lack evaluations on domains with various label-space sizes, \MyMethod demonstrates high scalability across different datasets and excels with a real-world pre-trained vision transformer on ImageNet-1k~\cite{caron2021emerging}.

% Except for controllable transferability, we draw comparisons between \MyMethod and existing NTL methods in Table~\ref{tab: comparison with baselines}. 
% Except for flexibility in controlling transferability, we present more limitations of existing NTL methods in Table~\ref{tab: comparison with baselines}.
% \MyMethod also overcomes the limitation of previous strategies over the robustness when the malicious users fine-tune the downstream models on unauthorized domains.
% Moreover, thanks to the sparse updating method, \MyMethod is more efficient and has less impact on the original encoder properties.
% Furthermore, we evaluate \MyMethod on various label-space sizes and across different data domains, 
% and also evaluate it on a real-world large image encoder--Vision Transformer--pretrained on ImageNet-1k by Facebook~\cite{caron2021emerging}.

% Model non-transferability for model Intellectual Property (IP) protection emerges as a nascent research topic, predominantly pivoting on whole-model optimization. 
% All methods gravitate towards a target-free learning scenario utilizing generative models, yet, diverging from the common use of Generative Adversarial Networks (GAN)~\cite{}, our approach aligns more closely with statistical meaning. \adam{what is "aligns with statistical meaning"?}
% Our strategy, along with the Model Barrier (MB)~\cite{wang2023model}, can be easily integrated with any DNN backbones. 
% However, \MyMethod, demanding only a handful of weight adjustments, minimally impacts the model's inherent properties. 
% Moreover, our experimental framework first explores fine-tuning various downstream classifiers and scenarios wherein the target domain exhibits a label space distinct from the source domain, thereby underlining the robustness and universality of \MyMethod.

% 

% \subsection{Multi-task Nontransferability} \label{sec: inductive-transfer-learning}
% Conventional Non-Transfer Learning intellectual property protection methods predominantly focus on scenarios where a pre-trained model is directly applied to a distinct data domain without additional fine-tuning.
% The Encoder-as-a-Service (EaaS) case, however, introduces additional complexities.
% A malicious client can query the service API using data from an unauthorized domain, fine-tuning downstream models for various tasks and essentially acting as an adaptive attacker against the NTL training scheme. 
% Therefore, defending against such adaptive attackers becomes imperative.
% This entails constraining the client's transferability for unauthorized tasks, especially with supervised fine-tuning, with varied label space sizes, or with different downstream model architectures, to adhere to predefined usage policies and preserve the integrity of the service.
 
\subsection{Preliminaries on Weight Vulnerability} \label{sec: inspiration dfa}



DNN fault attacks are built on the principle of identifying and modifying the vulnerable weight within a network~\cite{zhao2019fault,luo2021deepstrike, rakin2019bit}.
Guided by this understanding, our innovative technique, \MyMethod, enables meticulous control over encoder transferability by targeting a specific subset of weights.
Specifically, weights with higher absolute gradient values are often deemed vulnerable in DNN fault attacks, signifying their substantial influence on the model output. 
This characteristic gains prominence in transfer learning, involving data from both source and target domains.
We do a preliminary experiment on gradient values, illustrated in Figure~\ref{fig: motivation-dfa}.
Using a Multi-Layer Perceptron (MLP) of size (784-32-32-10), we train the model on the MNIST (source) and subsequently fine-tune the output layer on the USPS (target). 
The second hidden layer, representing the encoder API, consists of $32\times 32$ weights. 
Figure~\ref{fig: motivation-dfa} displays the gradient distribution for the hidden layer's weights in both source ({\color{red} Red}) and target ({\color{blue} Blue}) domains, revealing varied weight vulnerability across datasets.
\begin{table}[t]
    \caption{\textbf{Sparse weight update benefits---}including integrity, efficiency, versatility, flexibility.}
    \centering   
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{c|l}
    \toprule[0.6mm]
    Integrity   & Preserve original encoder functionality.\\
    Flexibility & Ease toggling between encoder modes. \\
    Versatility & Enable multi-level transferability.\\
    Efficiency  & Reduce computational cost during backpropagation.\\
    % Robustness  & Hinder overwriting through fine-tuning.\\
    \bottomrule[0.4mm]
    \end{tabular}
    }

    \label{tab: sparse weight update benefit}
\end{table}
Building upon this insight, we designed \MyMethod to selectively update critical weights for the target domain while preserving those relevant to the source domain.
Modifying only a fraction of the encoder's weights offers notable advantages in integration, flexibility, versatility, and computational efficiency, as detailed in Table~\ref{tab: sparse weight update benefit}. 
Primarily, \MyMethod seamlessly integrates with existing source domain encoders, enabling a faster training process with minimal source and target data. 
Furthermore, given the distinct weight vulnerability across data domains, sparse weight updating enhances adaptability to various unauthorized domains, enabling the creation of multi-level transferability.



\subsection{Design Criteria for \MyMethod} \label{sec: design objective}
In pursuing flexible controllability of the encoder's transferability, three design requirements should be satisfied: sparsity, effectiveness, and robustness.
\begin{enumerate}[leftmargin=*, itemsep=0pt, topsep=0pt]
\item \textbf{Sparsity Goal}: To uphold the original models' functionality as well as training efficiency, modifications should be confined to a limited set of weights. 
\item \textbf{Effectiveness Goal}: It's imperative that the encoder retains high accuracy in the source domain while exhibiting low accuracy in the target domain.
\item \textbf{Robustness Goal}: 
% Unlike in domain adaptation scenarios, malicious users in this setting can query the encoder for unauthorized features and train their own downstream models. 
This objective is to thwart the encoder's transferability even when the downstream classifier is malicious fine-tuned on the unauthorized domain.
\fei{what is the difference beween 3 and 2}
\ruyi{3 focus on the downstream classifier can be fine-tuned. 2 focus on a general goal for NTL.}
\end{enumerate}
